AvatarReX: Real-time Expressive Full-body Avatars

We present AvatarReX, a new method for learning NeRF-based full-body avatars from video data. The learnt avatar not only provides expressive control of the body, hands and the face together, but also supports real-time animation and rendering. To this end, we propose a compositional avatar representation, where the body, hands and the face are separately modeled in a way that the structural prior from parametric mesh templates is properly utilized without compromising representation flexibility. Furthermore, we disentangle the geometry and appearance for each part. With these technical designs, we propose a dedicated deferred rendering pipeline, which can be executed in real-time framerate to synthesize high-quality free-view images. The disentanglement of geometry and appearance also allows us to design a two-pass training strategy that combines volume rendering and surface rendering for network training. In this way, patch-level supervision can be applied to force the network to learn sharp appearance details on the basis of geometry estimation. Overall, our method enables automatic construction of expressive full-body avatars with real-time rendering capability, and can generate photo-realistic images with dynamic details for novel body motions and facial expressions.

==> sections/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}


Animatable human avatar modeling is of great importance in many applications such as content creation and immersive entertainment, and virtual characters have the potential to open up a new way for people to interact with others or intelligent machines in AR/VR settings. The classical pipeline for manually creating 3D human avatars involves tedious and time-consuming steps, including scanning, meshing, rigging and many more. Furthermore, such a pipeline requires expert knowledge and sophisticated capture systems, limiting its access and increasing its cost. 


In order to lower the entry barrier for novices and automate the workflow of experienced artists, researchers have devoted great efforts in learning 3D human avatars from images or videos of real humans. Building upon explicit meshes~\cite{timur2021driving_signal,habermann2021realtimeDDC}, implicit radiance fields~\cite{peng2021animatable_nerf,zheng2022structured} or both~\cite{Lombardi2021MVP,neural_actors,Remelli2022TexelAligned}, current approaches are able to synthesize realistic human motions under free-view points. Despite the plethora of these systems, most of them only model the torsos and the limbs, ignoring other fine-grained body parts like faces and hands~\cite{peng2021animatable_nerf,neural_actors}. To obtain expressive human avatars, however, we need the full controllability of the body, hands and the face, as the essential nuance of human behaviors is conveyed through a concert of body movements, hand gestures and facial expressions. 
Up to now, only research works from Meta Reality Lab are able to achieve this goal~\cite{timur2021driving_signal}. Unfortunately, their methods rely on video data captured from dense-view camera rigs, which is not accessible for most individuals and academic organizations. 


Apart from expressiveness, another unsolved challenge lies in the rendering speed. 
In many applications, the avatars are expected to interact with users as real human-beings, which emphasizes the need for real-time animation and rendering. 
However, the most recent approaches in this field are typically built upon neural radiance fields (NeRF)~\cite{mildenhall2020nerf}, which densely samples the 3D space and queries the network millions of times during volumetric rendering. Consequently, current state-of-the-art methods are difficult to animate the learnt avatar in interactive framerate, preventing them from being adopted in interactive scenarios.  
% To date there is no single approach to tackle both of these requirements.


% In this work, we present \textbf{R}eal-time \textbf{ex}pressive \textbf{Avatar} (AvatarRex), a novel system that simultaneously achieves expressive control and real-time animation of full-body human avatars.
% To this end, we propose a compositional yet light-weight representation, which models the face, hands and the body in tight accordance with their characteristics in shape and texture variations. %We further disentangle geometry and appearance for each part. 
% \textbf{(1) Body.} Considering the variety of clothing styles, we adopt the technique from ~\cite{zheng2022structured}, one of the state-of-the-art methods for body avatar modeling. This method makes no assumption on cloth topology and models the major body parts using a set of structured local radiance fields. To enhance its detail representation power, we equip each radiance field with a feature patch, allowing the network to store high-frequency appearance details in an explicit feature grid.
% \textbf{(2) Hand.}  For hand modeling, we observe that the shape variation of human hands is rather limited. Therefore, we directly build the radiance fields for both hands on top of the parametric hand template~\cite{Romero2017MANO}. 
% Such a design eliminates the need for learning thin structure and complex articulated motions of fingers using implicit neural representations, which is known to be a hard problem. 
% \textbf{(3) Face.}  Faces also follow a strong shape prior, but contain many more subtle yet important details relating to different expressions. 
% To faithfully represent the face avatar, we take advantage of the expression space of a 3D morphable model~\cite{wang2022faceverse}. 
% Specifically, we condition the facial radiance field on the orthogonal rendering of the morphable model, which serves as a dense signal of the facial expressions. In this way, our face avatar is able to generate high-fidelity images of various facial expressions. 

In this work, we present \textbf{R}eal-time \textbf{Ex}pressive \textbf{Avatar} (AvatarRex), a novel system that simultaneously achieves expressive control and real-time animation of full-body human avatars.
% To this end, we propose a  compositional avatar representation, which models the face, hands and the body with independent implicit neural field. 
% For each part, we further disentangle geometry and appearance, resulting into six implicit fields in total (Section~\ref{sec:avatar_reprez}). 
% Such a design allows us to adopt the best modeling method for each implicit field in tight accordance with its characteristics in shape or texture variations, as we briefly introduce in the following. 
To this end, we propose a compositional avatar representation, which models the face, hands and the body in tight accordance with their characteristics in shape and texture variations. %We further disentangle geometry and appearance for each part. 
\textbf{(1) Body.} Considering the variety of clothing styles, we adopt the technique from ~\cite{zheng2022structured} for body avatar modeling. This method makes no assumption on cloth topology and models the major body parts using a set of structured local radiance fields. To enhance its detail representation power, we equip each radiance field with a dynamic feature patch, which allows the network to store high-frequency appearance details in an explicit feature grid.
\textbf{(2) Hand.}  Considering that the shape variation of human hands is rather limited, we directly build the radiance fields for both hands on top of the parametric hand template~\cite{Romero2017MANO}. 
Such a design eliminates the need for learning thin structure and complex articulated motions of fingers using implicit neural representations, which is known to be a hard problem. 
\textbf{(3) Face.}  Faces also follow a strong shape prior, but contain many more subtle yet important details relating to different expressions. 
To faithfully represent the face avatar, we take advantage of the expression space of a 3D morphable model~\cite{wang2022faceverse}. 
Specifically, we condition the facial radiance field on the orthogonal rendering of the morphable model, which serves as a dense signal of the facial expressions. In this way, our face avatar is able to generate high-fidelity images of various facial expressions. 


With these building blocks at hand, we can now derive the final expressive avatar representation by assembling the face, hands and the body into one holistic model. However, it remains a challenge to combine different radiance fields together and render the final model efficiently.
To address these difficulties, we propose to utilize the signed distance field (SDF) as the common geometric representation. 
SDF can be either computed from a water-tight mesh or learned from data, allowing us to unify different body parts into one radiance field. 
Furthermore, we exploit the surface definition in SDF and propose a hybrid rendering method for training the networks. 
The key to our hybrid rendering method is to combine volume rendering and surface rendering. 
% Specifically, we perform volume rendering through sampling and integrating along camera rays, as done in NeRF~\cite{mildenhall2020nerf}. For surface rendering, we first extract the iso-surface from the SDF and only render the intersection points between the camera rays and the surface. 
Volume rendering makes it possible to learn various cloth shape and topology from video data, while surface rendering minimizes network queries, enabling perceptual supervision on image patches. 
Once network training is done, we directly perform surface rendering for animation, which can be executed in real-time framerate with our dedicated deferred shading pipeline.  

% With these building blocks at hand, we can now derive the final expressive avatar representation by assembling the face, hands and the body into one holistic model. 
% However, it remains a challenge to learn an avatar model with sharp appearance details and render it efficiently. 
% To resolve the these problem, we further improve our avatar representation by disentangling the geometry and appearance for each part and using the signed distance field (SDF) as the common geometric representation. 



% \textbf{(1)}  
% \textbf{(2)} 
% \textbf{(3)} 






% In this work, we aim to simultaneously achieves expressive control and real-time animation of full-body human avatars.
% This is a difficult target,  as it requires us to not only take into account the  body parts, but also make the system as light-weight as possible. 
% Having this in mind, we design a novel hybrid representation, which models the face, hands and the body in tight accordance with their characteristics in shape and texture variations.



In summary, our system is able create expressive, photo-realistic full-body avatar that can be animated and rendered in real time. 
Given the video data captured from 22 cameras (16 for the body, 6 for the face), our network can be trained in an end-to-end manner, without any pre-scanning efforts or other manual assistance or intervention. After network training, the avatar can be driven in real-time given new body poses, hand gestures and facial expressions. Experimental results clearly show the potential of applying our method in interactive applications. 


